SparGE: Sparse Coding-based Patient Similarity Learning via Low-rank Constraints and Graph Embedding

Patient similarity assessment (PSA) is pivotal to evidence-based and personalized medicine, enabled by analyzing the increasingly available electronic health records (EHRs). However, machine learning approaches for PSA has to deal with inherent data deficiencies of EHRs, namely missing values, noise, and small sample sizes. In this work, an end-to-end discriminative learning framework, called SparGE, is proposed to address these data challenges of EHR for PSA. SparGE measures similarity by jointly sparse coding and graph embedding. First, we use low-rank constrained sparse coding to identify and calculate weight for similar patients, while denoising against missing values. Then, graph embedding on sparse representations is adopted to measure the similarity between patient pairs via preserving local relationships defined by distances. Finally, a global cost function is constructed to optimize related parameters. Experimental results on two private and public real-world healthcare datasets, namely SingHEART and MIMIC-III, show that the proposed SparGE significantly outperforms other machine learning patient similarity methods.

==> back.tex <==
\begin{comment}
\cite{suo2018multi_icdm} 
Data of different physical properties, their units of measurement are also different, for example, age and blood pressure. It is difficult to find the  correlation between data having different units, for example, age and LV mass. Furthermore, it is not easy to explicitly perform sparse feature selection for existing multi-task metric learning models, and as the feature dimension increases, the dimensions of the Mahalanobis matrix increase, which may cause the over-fitting issue.


%
Compared to state of the art  \emph{TDDL}  methods, the proposed \emph{SparGE} framework
shares the following three merits:



% \cite{wang2019measurement_beo} Many previous studies usually calculated the patient similarity using single similarity measures 
% (e.g., Euclidean distance, cosine distance, and Mahalanobis distance), and most of them did not take the importance of patient features into consideration while calculating the similarity. 
% In this study, we aimed to investigate in depth the patient similarity in the following two aspects.
% One is using different similarity metrics for different types of feature data. 
% The other is assigning different weights (importance) to patient features when integrating feature similarities into a patient similarity.

% %
% \paragraph{outline3: concludes traditional methods and however}
% %
% Although predictor extraction affects the performance of the model [24], one of the challenging tasks 
% in patient similarity-based predictive modeling is identifying the most relevant and important patient characteristics for patient similarity assessment. 

% Existing methods have successfully derived the similarity measure from EHR data through mapping the medical events into vector spaces, 
% however, their applicability is limited due to the lack of convincing explanations for patient representations in medical domain.
% There has been some existing work on applying patient similarity to various applications in medical literatures. 
% However, there are still significant challenges on learning effective patient similarities, which, to our knowledge, have not been systematically addressed.
% %%%=============================================================%%%
% %%                           SECTION 1.2                         %%
% %%%=============================================================%%%    


% %%%=============================================================%%%
% %%                          SECTION 1.2                           %%
% %%%=============================================================%%%
% \subsection{Paper Structure and Notations} 
% %
% The rest of this paper is organized as follows. 
% %Section \ref{sec:02} provides an overview of related work.
% %Section~\ref{sec:02} provides a brief review on both sparse representations and the trace quotient optimization.
% %
% In Section \ref{sec:02}, we provide a brief introduction of sparse representations and then investigate its sample complexity.
% %
% %smooth locality-constrained dictionary learning and then investigate its differentiability.
% %and then develop its differentiable version. % for both unsupervised and supervised setting. 
% %We begin with a brief review of related work in DR models in .   derive
% %
% In Section~\ref{sec:03}, we propose a generic cost function that learns a sparsifying dictionary and orthogonal transformations.
% %and then discuss its several exemplifications in Section~\ref{sec:04}.
% A geometric stochastic gradient algorithm is developed in Section~\ref{sec:04},
% %
% %The development of a gradient descent algorithm is also discussed in this section. % also
% %An extended DR approach via multi-layer coupled dictionary learning is described in Section \ref{sec:04}. % \ref{sec:04} also derive also
% % Section \ref{sec:06} describes the development of a conjugate gradient algorithm and
% %% The development of a conjugate gradient algorithm is discussed in this Section \ref{sec:05}. % also
% Section \ref{sec:05} presents the implementation settings and simulational experiments.
% % for images DR, classification, and local features coding. 
% Finally, we draw the conclusion of our work in Section \ref{sec:06}.  
% %Finally, conclusions and outlook are given in Section~\ref{sec:07}.


% In this work, vectors and matrices are denoted by bold lower case letters and upper case ones, respectively. 
% %   
% $\bm{I}_n$ denotes $n\times n$-identity matrix, 
% $\mathbf{1}_k$ denotes the $k$ dimensional all-ones column vector, 
% $\mathbf{1}_{k\times k}$ denotes the $k\times k$ all-ones square matrix, 
% $\|\cdot\|_F$  denotes the Frobenius norm of matrices,  
% $\bm{v}_i$ denotes the $i^{th}$ column of matrix $\bm{\mathcal{V}}$,
% $\bm{E}_{ij}$ denotes the matrix whose $i^{th}$ entry in the $j^{th}$ column equals to one, and all other entries are zero,
% $\operatorname{tr}(\cdot)$ denotes the trace of a matrix,
% $\bm{v}_i$ denotes the $i^{th}$ column of matrix ${\mathbf{U}}$,
% and,
% $\mathcal{R} (\cdot)$ denotes the full vector of a sparse representation. 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%                           SECTION 2                           %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Related Work}
% \label{sec:02}
% Most commonly, through exhaustive comparisons between a given patient and a cohort of existing patients, an assessment specific to the given patient can help in identifying his similar patients. 

% The traditional predictive modelling approach involves building a global predictive model using all available training data. 
% However, this may not be the most suitable approach for personalized prediction for individual patients.
% In this context \cite{}, individualized predictive modelling based on patient similarity emerged and was shown to be adjustable for individual patients. 

%\subsection{clustering based methods}
%



%\subsection{metric learning based methods}
%


%\subsection{feature selection based methods}
%

%\subsection{sparse and low-rank based methods}
%

%
%\subsection{Comparison and the advantages}
%

\end{comment}
